Learning Robust Hierarchical Patterns of Human Brain across Many fMRI Studies

Resting-state fMRI has been shown to provide surrogate biomarkers for the analysis of various diseases. In addition, fMRI data helps in understanding the brain's functional working during resting state and task-induced activity. To improve the statistical power of biomarkers and the understanding mechanism of the brain, pooling of multi-center studies has become increasingly popular. But pooling the data from multiple sites introduces variations due to hardware, software, and environment. In this paper, we look at the estimation problem of hierarchical Sparsity Connectivity Patterns (hSCPs) in fMRI data acquired on multiple sites. We introduce a simple yet effective matrix factorization based formulation to reduce site-related effects while preserving biologically relevant variations. We leverage adversarial learning in the unsupervised regime to improve the reproducibility of the components. Experiments on simulated datasets display that the proposed method can estimate components with improved accuracy and reproducibility. We also demonstrate the improved reproducibility of the components while preserving age-related variation on a real dataset compiled from multiple sites.

==> dataset_table.tex <==
\begin{table}[h!]
\centering
\begin{tabular}{ llllll }
 \hline

Data Sites & No. of Participants  & Age Range (Median) & Similarity with pooled components\\
 \hline
 BLSA-3T    & $784$  & $[22,95](68)$ & $0.6136$\\
 CARDIA\_1   & $199$   & $[42,61](52)$ & $0.5902$\\
 CARDIA\_3   & $321$  & $[43,61](52)$ & $0.5636$\\
 CARDIA\_4   & $278$   & $[43,62](52)$ & $0.5470$\\
 UKBB  & $2023$&  $[45,79](63)$ & $0.6518$\\
OASIS    & $847$ &$[42.6,97](70)$ & $0.6316$\\
ADC   & $279$ &  $[23,95](70)$ & $0.5264$\\
 \hline

\end{tabular}
 \caption{Summary characteristics of the datasets. Last column shows similarity of the components derived from individual sites with the components derived from the pooled dataset. We can see that sites having larger sample size have more similarity with the components derived from the pooled dataset. \textbf{Todo}: Show age distribution}
 \label{fig:summary}
\end{table}


==> new_dataset_table.tex <==
\begin{table}[t!]
 \caption{Summary characteristics and age range along with the median is shown for each data site.}
 \label{tbl:summ}
\centering
\begin{minipage}[t]{0.45\linewidth}
\begin{tabular}[t]{ ccc}
 \hline

Data Site & Participants  & Age Range \\
 \hline
 BLSA-3T    & $784$  & $[22,95](68)$ \\
 CARDIA\_1   & $199$   & $[42,61](52)$ \\
 CARDIA\_3   & $321$  & $[43,61](52)$ \\
 CARDIA\_4   & $278$   & $[43,62](52)$ \\
 \hline

\end{tabular}
\end{minipage}
\hfill
\begin{minipage}[t]{0.45\linewidth}
\begin{tabular}[t]{ ccc }
 \hline

Data Site & Participants  & Age Range\\
 \hline
UKBB  & $2023$&  $[45,79](63)$\\
OASIS    & $847$ &$[42.6,97](70)$ \\
ADC   & $279$ &  $[23,95](70)$ \\
 \hline

\end{tabular}
\end{minipage}

\end{table}

==> tables/25_new.tex <==
        \begin{center}


        \begin{tabular}{ |p{2cm}||p{2.3cm}|p{2.3cm}|p{2.3cm}|p{2.3cm}|  }
 \hline
 \multicolumn{5}{|c|}{Comparison by varying sparsity parameter (components = 25)}\\
 \hline
\% non-zeros &  0.9671 & 0.9057  & 0.6824 &  0.3776\\ 
 \hline
 Reproducibility   & $0.6042 \pm 0.0185$    & $0.6296 \pm 0.0110 $ &   $0.5952 \pm 0.0336 $ & $0.6004 \pm 0.0254 $ \\
 \hline
\end{tabular}
            
        \end{center}


==> tables/age_prediction.tex <==
        \begin{center}


        \begin{tabular}{ |p{2cm}||p{2.3cm}|p{2.3cm}|p{2.3cm}|p{2.3cm}|  }
 \hline
 \multicolumn{5}{|c|}{Comparison by varying sparsity parameter (components = 25)}\\
 \hline
\% non-zeros &  0.9431 & 0.8625  & 0.6751 &  0.3967\\ 
 \hline
 MAE   & $9.1754 \pm 1.15$    & $ 9.2055 \pm 1.2194 $ &   $9.1915 \pm 1.2247 $ & $9.2240 \pm 1.1220 $ \\
 \hline
\end{tabular}
            
        \end{center}

==> tables/corr_h1.tex <==
\begin{table}[t!]
\caption{Mean absolute error \label{tbl:corr_h1}}
\centering
        \begin{tabular}{ ccccc }
 %\hline
 %\multicolumn{5}{|c|}{Comparison by varying number of components}\\
 \toprule
 {Method} & {$k_1=10$} & {$k_1=15$}  & {$k_1=20$} & {$k_1=25$} \\
 \midrule
hSCP & $0.641\pm0.029$   & $0.633\pm0.009$   &  $0.626\pm0.012$ &   $0.610\pm0.022$\\
Adv. hSCP & $0.664\pm0.028$ &  $0.650\pm0.021$  &  $0.647\pm0.023$ &    $0.638\pm0.019$ \\
Mod. hSCP & $0.752\pm0.024$ &   $0.716\pm0.021$ &    $0.688\pm0.014$ &   $0.692\pm0.018$ \\
Adv. + Mod. hSCP & $0.759\pm0.026$ & $0.722\pm0.025$ & $0.696\pm0.019$ &  $0.694\pm0.022$ \\
 \bottomrule
\end{tabular}
\end{table}

==> tables/corr_h2.tex <==
\begin{table}[t!]
\caption{Mean absolute error \label{tbl:corr_h2}}
\centering
        \begin{tabular}{ ccccc }
 %\hline
 %\multicolumn{5}{|c|}{Comparison by varying number of components}\\
 \toprule
 {Method} & {$k_1=10$} & {$k_1=15$}  & {$k_1=20$} & {$k_1=25$} \\
 \midrule
hSCP & $0.641\pm0.029$   & $0.633\pm0.009$   &  $0.626\pm0.012$ &   $0.610\pm0.022$\\
Adv. hSCP & $0.664\pm0.028$ &  $0.650\pm0.021$  &  $0.647\pm0.023$ &    $0.638\pm0.019$ \\
Mod. hSCP & $0.752\pm0.024$ &   $0.716\pm0.021$ &    $0.688\pm0.014$ &   $0.692\pm0.018$ \\
Adv. + Mod. hSCP & $0.759\pm0.026$ & $0.722\pm0.025$ & $0.696\pm0.019$ &  $0.694\pm0.022$ \\
 \bottomrule
\end{tabular}
\end{table}

==> tables/h_simu_accu.tex <==
\begin{table}[t!]
\caption{Accuracy on simulated dataset \label{tbl:h_simu_accu}}
\centering
        \begin{tabular}{ llllll }
 %\hline
 %\multicolumn{5}{|c|}{Comparison by varying number of components}\\
 \toprule
 & {Method} & {$k_1=8$} & {$k_1=10$}  & {$k_1=12$} & {$k_1=14$} \\
 \midrule
\multirow{ 4}{*}{$k_2=4$} & hSCP & $0.789$    & $0.787$ &   $0.745$ & $0.736$\\
& Adv. hSCP & $0.869 $     & $0.875$ &  $0.862$  & $0.854$ \\
& Mod. hSCP & $0.873 $     & $0.865$ &  $0.843$  & $0.867$ \\
& Adv. + Mod. hSCP & $ 0.903 $     &$0.910$  &  $0.902$  &  $0.908$\\
\midrule
\multirow{ 4}{*}{$k_2=4$} & hSCP & $0.789$    & $0.787$ &   $0.745$ & $0.736$\\
& Adv. hSCP & $0.869 $     & $0.875$ &  $0.862$  & $0.854$ \\
& Mod. hSCP & $0.873 $     & $0.865$ &  $0.843$  & $0.867$ \\
& Adv. + Mod. hSCP & $ 0.903 $     &$0.910$  &  $0.902$  &  $0.908$\\
 \bottomrule
\end{tabular}
\end{table}

==> tables/h_simu_repro.tex <==
\begin{table}[t!]
\caption{Reproducbility on simulated dataset \label{tbl:h_simu_repro}}
\centering
        \begin{tabular}{ lllll }
 %\hline
 %\multicolumn{5}{|c|}{Comparison by varying number of components}\\
 \toprule
 {Method} & {$k_1=8$} & {$k_1=10   $}  & {$k_1=12$} & {$k_1=14$} \\
 \midrule
hSCP & $0.769\pm0.052$    & $0.798 \pm 0.047$ &   $0.739 \pm 0.053$ & $0.734 \pm 0.047$\\
Adv. hSCP & $0.781 \pm 0.037$     & $0.828 \pm 0.030$ &  $0.780 \pm 0.034$  & $0.750 \pm 0.031 $ \\
Mod. hSCP & $0.825 \pm 0.039$     & $0.845\pm 0.030$ &  $0.826\pm 0.039$  & $0.779\pm 0.366$ \\
Adv. + Mod. hSCP & $ 0.840 \pm 0.044$     &$0.869 \pm 0.034$  &  $0.815 \pm 0.035$  &  $0.802 \pm 0.030$\\
 \bottomrule
\end{tabular}
\end{table}

==> tables/scan_comparison.tex <==
        \begin{tabular}{ |p{2cm}||p{1.5cm}|p{1.5cm}|p{1.5cm}|p{1.5cm}|  }
 \hline
 \multicolumn{5}{|c|}{Similarity}\\
 \hline
& BLSA & CARDIA\_1  & CARDIA\_3 & CARDIA\_4\\
 \hline
 BLSA   & 1    & 0.840 & 0.713 & 0.712\\
 CARDIA\_1 & 0.840  & 1   & 0.770 & 0.839\\
CARDIA\_3    & 0.713 & 0.770  & 1 & 0.883\\
 CARDIA\_4 & 0.712 & 0.839  & 0.883 &1\\
 \hline
\end{tabular}

==> tables/scanner_effect.tex <==
                \centering

        \begin{tabular}{ |p{2cm}||p{2.3cm}|p{2.3cm}|p{2.3cm}|p{2.3cm}|p{2.3cm}|  }
 \hline
 \multicolumn{6}{|c|}{Comparison by varying sparsity parameter (components = 10)}\\
 \hline
& 0.001 & 0.1 &0.5 &1 &5\\
 \hline
 Reproducibility   & $0.8552 \pm 0.0387$    & $0.8481 \pm 0.0576$ &   $0.9158 \pm 0.0308$ & $0.8841 \pm 0.0617$ & $0.8816 \pm 0.0477$ \\
 Information ratio & $0.7814 \pm 0.0097$  & $1.0882 \pm 0.003$   & $1.3317 \pm 0.003$ & $1.4283 \pm 0.0019$ & $1.428 \pm 0.0022$\\
 AUC &  $0.5911 \pm 0.0377$ &    $0.6167 \pm 0.0251$    &    $0.6545 \pm 0.0139$  &  $0.6442 \pm 0.0168$ & $0.6402 \pm 0.0248$\\
 \hline
\end{tabular}

==> tables/scanner_effect_25.tex <==
                \centering

        \begin{tabular}{ |p{2cm}||p{2.3cm}|p{2.3cm}|p{2.3cm}|p{2.3cm}|p{2.3cm}|  }
 \hline
 \multicolumn{6}{|c|}{Comparison by varying sparsity parameter (components = 25)}\\
 \hline
& 0.001 & 0.1 &0.5 &1 &5\\
 \hline
 Reproducibility   & $0.8577 \pm 0.0389$    & $0.8805 \pm 0.0306 $ &   $0.8309 \pm 0.0450 $ & $0.8213 \pm 0.0601 $ & $0.8319 \pm 0.0595$ \\
 Information ratio & $1.0077 \pm 0.0075$ &  $1.0530 \pm 0.0066$  &  $1.2737 \pm 0.0030$ &   $1.6017 \pm  0.0032$&       $1.6131 \pm 0.0019$\\
 AUC &  $0.6033 \pm 0.0260 $ &    $0.6357 \pm 0.0263 $    &    $0.6664 \pm 0.0343 $  &  $0.6596 \pm 0.0284 $ & $0.6572 \pm 0.0215 $\\
 \hline
\end{tabular}

==> tables/split_sample.tex <==
        \begin{center}


        \begin{tabular}{ |p{2cm}||p{2.3cm}|p{2.3cm}|p{2.3cm}|p{2.3cm}|  }
 \hline
 \multicolumn{5}{|c|}{Comparison by varying sparsity parameter (components = 25)}\\
 \hline
\% non-zeros &  0.9320 & 0.8751  & 0.6929 &  0.4223\\ 
 \hline
 Reproducibility ($\mathbf{W}$)  & $0.6919 \pm 0.0191$    & $0.7034 \pm 0.0210 $ &   $0.6881 \pm 0.0213 $ & $0.6892 \pm 0.0198 $ \\
  Reproducibility ($\mathbf{D}$)  & $0.7644 \pm 0.0344$    & $0.8127 \pm 0.0228 $ &   $0.8210 \pm 0.0317 $ & $0.8633 \pm 0.0140 $ \\
 \hline
\end{tabular}
            
        \end{center}

==> tables/table_real_repro.tex <==
\begin{table}[t!]
\caption{Split-sample reproducbility on real dataset at one level \label{tbl:real_repro}}
\centering
        \begin{tabular}{ ccccc }
 %\hline
 %\multicolumn{5}{|c|}{Comparison by varying number of components}\\
 \toprule
 {Method} & {$k_1=10$} & {$k_1=15$}  & {$k_1=20$} & {$k_1=25$} \\
 \midrule
hSCP & $0.641\pm0.029$   & $0.633\pm0.030$   &  $0.626\pm0.012$ &   $0.610\pm0.022$\\
Adv. hSCP & $0.664\pm0.028$ &  $0.650\pm0.021$  &  $0.647\pm0.023$ &    $0.638\pm0.019$ \\
Mod. hSCP & $0.752\pm0.024$ &   $0.716\pm0.021$ &    $0.688\pm0.014$ &   $0.692\pm0.018$ \\
Adv. + Mod. hSCP & $\mathbf{0.754\pm0.026}$ & $\mathbf{0.721\pm0.025}$ & $\mathbf{0.689\pm0.019}$ &  $\mathbf{0.694\pm0.022}$ \\
 \bottomrule
\end{tabular}
\end{table}


           


       




           



==> tables/table_simu.tex <==
\begin{table}[t!]
\caption{Accuracy and Reproducbility on simulated dataset \label{tbl:simu_accu_new}}
\centering
        \begin{tabular}{ lllllllll }
        &  \multicolumn{4}{c}{Accuracy}     & \multicolumn{4}{c}{Reproducibility}              \\
    \cmidrule(r){2-5} \cmidrule(r){6-9}
 %\hline
 %\multicolumn{5}{|c|}{Comparison by varying number of components}\\
 {Algo.} & {$8$} & {$10$}  & {$12$} & {$14$} & {$8$} & {$10$}  & {$12$} & {$14$}\\
 \midrule
(a) & $0.789$    & $0.787$ &   $0.745$ & $0.736$ & $0.769\pm0.052$    & $0.798 \pm 0.047$ &   $0.739 \pm 0.053$ & $0.734 \pm 0.047$ \\
(b) & $0.869 $     & $0.875$ &  $0.862$  & $0.854$& $0.781 \pm 0.037$     & $0.828 \pm 0.030$ &  $0.780 \pm 0.034$  & $0.750 \pm 0.031 $ \\
(c) & $0.873 $     & $0.865$ &  $0.843$  & $0.867$ & $0.825 \pm 0.039$     & $0.845\pm 0.030$ &  $0.826\pm 0.039$  & $0.779\pm 0.366$ \\
(d) & $ 0.903 $     &$0.910$  &  $0.902$  &  $0.908$ & $ 0.840 \pm 0.044$     &$0.869 \pm 0.034$  &  $0.815 \pm 0.035$  &  $0.802 \pm 0.030$\\
 \bottomrule
\end{tabular}
\end{table}
